Emotional Strain and Frustration in LLM Interactions in Software Engineering

Large Language Models (LLMs) are increasingly integrated into various daily tasks in Software Engineering such as coding and requirement elicitation. Despite their various capabilities and constant use, some interactions can lead to unexpected challenges (e.g. hallucinations or verbose answers) and, in turn, cause emotions that develop into frustration. Frustration can negatively impact engineers' productivity and well-being if they escalate into stress and burnout. In this paper, we assess the impact of LLM interactions on software engineers' emotional responses, specifically strains, and identify common causes of frustration when interacting with LLMs at work. Based on 62 survey responses from software engineers in industry and academia across various companies and universities, we found that a majority of our respondents experience frustrations or other related emotions regardless of the nature of their work. Additionally, our results showed that frustration mainly stemmed from issues with correctness and less critical issues such as adaptability to context or specific format. While such issues may not cause frustration in general, artefacts that do not follow certain preferences, standards, or best practices can make the output unusable without extensive modification, causing frustration over time. In addition to the frustration triggers, our study offers guidelines to improve the software engineers' experience, aiming to minimise long-term consequences on mental health.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> notes.tex <==
Notes from the Main start here


\section{Introduction}



%Background Information

%Problem Statement 

%Specific Focus and RQs

%Why is this Research Important?


%Overview of the Paper








When do software engineers feel frustrated when using LLMs?
* when using it for references
What the reason or source of frustration?
* e.g., get incorreect answers
How do they deal with frustration?
* e.g., change prompt, google the answer, give up 
How can the experience be less frustrating?
* improvements, 
How can the frustrating experience impact motivation?





\section{Background}
% what is frustration 

Software developers, moods, emotions,
and performance

"Wrobel	[13] conducted	a	survey	with	49	participants,	which showed that	developers	feel a	broad	range	
of	affects	while	programming—all	the affects	of	the	measurement	instrument’s	spectrum. Positive	
affects	are	perceived	to	be	those	enhancing	their	productivity. Frustration is	the	negative	affect	more	
often	felt,	as	well	as	the	one	perceived	as	deteriorating productivity"

https://arxiv.org/pdf/1405.4422

survey about AI and its impact

%%https://www.theregister.com/2024/07/26/ai_hinders_productivity/#:~:text=Some%2047%20percent%20of%20workers,productive%20while%20increasing%20their%20workload.



% frustrations in dialogues


\textbf{Techno-frustration}

Technostrain describes the immediate reaction from working with ICTs (Salanova et al., 2013), which can be perceived on a behavioral, psychological, and physiological level (Weinert et al., 2020). Thus, technostrain is commonly described as a multi-facetted construct that not only includes acute reactions to technology-based stressors, but also describes any negative effects that ICT-use has on humans (Nisafani et al., 2020). Psychological strain is often defined as techno-exhaustion (Ayyagari et al., 2011), which describes a feeling of being tired, fatigued, and frustrated by ICT-use (Weinert et al., 2020). In our study, we mainly focus on techno-frustration as a facet of psychological technostrain, describing the feeling of being uncertain, discouraged, confused, stressed, and upset due to ICT-use. Thus, IO and techno-frustration focus both on consequences of ICT-use. While IO measures the impact of ICT-use on people's experience of being overwhelmed by complex, ambiguous or too much information, the concept of techno-frustration captures the negative affective consequences that arise from those experiences. Consequences of psychological strain include, for example, decreased job satisfaction or the increased risk of burnout (Srivastava et al., 2015). \cite{muller2023can}
\url{https://www.sciencedirect.com/science/article/pii/S0747563222002606}



Moreover, research on information processing (Markus, 1990) indicates that frustration redirects “limited attentional resources away from the central task or goal at hand to peripheral features of the information environment that may now have become obstacles” (Bessière et al., 2006, p. 944).\cite{novak2022frustration}


communication patterns influence user’s perception, frustration, and harassment behavior \cite{brendel2020you}



On the contrary, frustration, anxiety, and confusion arise when there are obstructions in the interaction, and these are appraised as incongruent with the goals of the user. The relation of emotional user experience to interaction events can be analysed with the bipolar competence–frustration model, in which feelings of competence (or techno-competence) arise from successful task completion and the users perceiving their own skills in a positive light, whereas, frustration (or techno-frustration) is the result of being obstructed and unable to accomplish task goals (Saariluoma and Jokinen, 2014). \cite{jokinen2015emotional}



Lack of true understanding – LLMs don’t really “get” subtext
LLMs don’t really understand language the same way humans do. They are very skilled at statistically mimicking the patterns of human communication. But they lack the rich contextual knowledge, commonsense reasoning, and theory of mind that allows humans to fluently interpret subtext, tone, analogies, sarcasm, and implicit meanings.

For example, if you sarcastically said to an LLM “Well that’s just great!”, intending to convey frustration, the LLM might incorrectly interpret it as positive sentiment and respond with a chipper “I’m glad you’re happy!”. Or if you make an analogy or reference that isn’t in its training data, e.g. “That’s like finding a needle in a blueberry pie”, it will get very confused.

%Where are the expectations coming from?

In some cases, expectations are set by the users themselves, governed by internal sources, like prior experience with the technology. Noyes and Starr (Citation2003) learned that flight deck crews with no experience flying with automated warning systems tended to have more negative expectations of the technology, whereas their experienced counterparts tended to have expectations that were more positive of the automated warning system. This is understandable as the individuals with no experience have no basis of reference for how the warning system will perform. This may add an additional layer to the interaction where trust is involved. Without prior experience, these individuals likely were less trustworthy of the technology, and therefore developed more negative expectations for it. Conversely, those who have used the warning system before have a repository of experiences to reference, reducing the likelihood that something unexpected may catch them off guard. Additionally, their prior experience offers them more knowledge in what to expect, therefore having more positive views of the technology.

In other cases, expectations originate from an external source, such as the company responsible for the product. Roscoe et al. (Citation2017) designed a study to prime participants’ initial expectations of an automated writing system by describing it as either well-established or under development to influence expectations to be high or low, respectively. Interestingly, when asked about the likelihood that they would recommend the technology to someone else, individuals who were primed to have a more positive expectation of the technology, were less likely to recommend it. It is possible that the automated writing system did not meet their expectations when it came time for them to use it. This can serve as a cautionary tale to manage expectations with a product’s actual capabilities so as not to lead individuals too strongly in one direction or the other. It would be safer to slightly undersell the product, as opposed to promising perfection, risking that individuals’ expectations are too high and then not met. Overall, this highlights the impact that internal or external expectations prior to actual use of a system can have on attitudes and behaviours following use.

https://www.tandfonline.com/doi/full/10.1080/1463922X.2022.2095458#d1e145




Hadlington and Scase (Citation2018) considered individual differences in responses to technology failures, relating specifically to personality. 

\section{Methodology}
% write about the observational study
% talk about how we identify frustrations (IPA)
% qualitative analysis to identify the causes, how people react



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/method.pdf}
    \caption{The process we followed to conduct our study.}
    \label{fig:method}
\end{figure}

\textbf{Survey}



Demographics:

Age
gender (maybe)
field
technical proficiency on LLMs


Part 1
what LLMs do you use
how often
what purpose
how high are your expectations for the accuracy of responses from LLMs?
how often do you encounter incorrect or unsatisfactory answers from LLMs?
what is your initial reaction when you receive an incorrect answer from an LLM? (frustrated, annoyed, indifferent, amused, curious,...)
how intense? (not sure about this one)
what do you typically do after receiving an incorrect answer from an LLM?
how likely are you to provide feedback on incorrect answers to improve the LLM?
how has your trust in LLMs been affected by incorrect answers?
are you more or less likely to use LLMs in the future based on your experiences with incorrect answers?

Open questions:

what annoys you more when using LLMs?
Describe a situation where the response from an LLM did not meet your expectations. What did you expect and what was the actual response?
Describe a specific incident where an LLM gave you an incorrect answer and your reaction to it.
What improvements would you like to see in LLMs to reduce the occurrence of incorrect answers?
How do you think LLMs can better handle user frustration when they provide incorrect answers?


Psychometric tool to measure frustration (needs to be adapted)

Extension of the BIS/BAS scales 
1	2	3	4	5	6	Item-total

When circumstances prevent me from achieving an important goal, I find it hard to keep trying 
When an event I am looking forward to is cancelled, I lose the energy to arrange an alternative 
When I don’t get what I want, I lose interest in my day-to-day tasks 
If I have been working hard at something I lose motivation if I don’t get the reward I deserve 
When something good I am expecting doesn’t happen, I feel less enthusiastic about life for a while

https://doi.org/10.1016/j.paid.2009.06.015

\begin{table}[h]
  \caption{Survey Questions}
  \centering
  \begin{tabular}{p{0.95\linewidth}}
    \hline \hline
    \textbf{Question} \\ \hline
    Do you agree to participate in the survey and for us to use the data you provide for research anonymously? \\[1ex]
    1. What is your age? \\[1ex]
    2. What is your role? \\[1ex]
    3. What is your organisation's domain? (industry/academia) \\[1ex]
    4. How familiar are you with Large Language Models (LLM)? \\[1ex]
    5. How often do you use LLMs at work? \\[1ex]
    6. Briefly describe what LLMs you use and for what purpose in your work. \\[1ex]
    7. Write three expectations from LLMs that are most important for you when using them at work. \\[1ex]
    8. Explain how you feel when you receive an incorrect answer from an LLM? \\[1ex]
    9. What do you typically do after receiving an incorrect answer from an LLM? \\[1ex]
    10. Describe how your motivation to continue your task is affected if your interaction with the LLM did not assist you as intended with that task. \\[1ex]
    11. Describe a situation where you felt frustrated when using LLMs. What did you expect and what was the actual response? \\[1ex]
    12. What improvements would you like to see in LLMs to make the experience less frustrating? \\[1ex]
    13. Rate how important each of these factors is in leading to a frustrating experience (Hallucination, Intention not understood, Performance issues (e.g., LLM's server is down), Incorrect responses, LLM refuses to answer (e.g., "As a Large Language Model I cannot answer that ...")). \\ \hline
  \end{tabular}
  \label{tab:survey_questions}
\end{table}

\section{Results}

We identify dialogues with potential frustration  in Table \ref{tab:frst_summary} by observing an indication in the dialogue logs as a follow-up on a response (for example, asking the same question more than two times while getting the same answer), or a direct mention of frustration with a link to a specific conversation in the survey.
There are some conversations with "negative" feedback such as "The code you provided does not work". But we do not consider these as frustrations.


\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{2cm}p{6cm}p{5cm}p{3cm}}
    \toprule
        Participant No. & Frustration indication (Survey) & Frustration indication (Chats) & Reason of frustration \\
    \midrule
        1008 & Unfortunately I experienced alot of performance issues. It is quite long response time and sometimes the answers are aborted in the middle of a sentance or code. This makes it hard to use from time to time. Also it seems that there is a limit when it comes to  & "This doesn't work!" - keeps asking for a complete solution but not getting any. (20-3-2023\_1\_1008.mhtml) & Performance problems, limited generated tokens \\
        
        2010 & Frustrating. Even though ChatGPT confidently gives an answer to my questions, it was always unclear how it got to that answer, so I asked it for sources but then it gave me sources that were unrelated to my query, so I still did not know if the answer I got was in any way correct. Usually it was not. & Refers to the conversation mentioned in the survey (20230331\_2010.mhtml) & Source is not provided. Version not considered. \\
        2013 & "the responses given might be utter nonsense." - "cannot trust the information that ChatGPT spits out" & One-tab action dialogues: (29-03-2023\_1\_2013.mhtml / 29-03-2023\_2\_2013.mhtml / 29-03-2023\_3\_2013.mhtml / 29-03-2023\_4\_2013.mhtml) & Intent not understood \\
        4019 & "Go on Google, test out the actual code or solution, then reach the crushing realization that it is actually not true." & "also im disappointed in you" for not understanding intent (27\_4\_2023\_2\_4019.mhtml) & Intent not understood \\
        7035 & "GPT wrote me instructions which looks like valid. I followed them and found that the instructions were not valid." & refers to the dialogue in the survey (29-05-2023\_1\_7035.mhtml) &  Hallucination \\
        3020 & N/A & Asking to generate novel idea: (27-4-2023\_1\_3020.mhtml) & Unable to provide the requested response \\
    \bottomrule
    \end{tabular}
    \caption{Summary of the participants with identified frustrations and the corresponding reason.}
    \label{tab:frst_summary}
\end{table*}



\subsection{Causes of frustrations}
% also include how people usually react to frustration


\subsection{Answers to survey questions}

\textcolor{blue}{Q12 What improvements would you like to see in LLMs to make the experience less frustrating?}

\textcolor{blue}{When asked about the improvements participants would like to see in large language models (LLMs) to reduce frustration, several aspects emerged consistently from both groups' responses, showing shared frustrations and desired improvements, particularly around accuracy, transparency, and prompt understanding. See Figure \ref{fig:Q12}
Transparency: Participants expressed a need for LLMs to be transparent about their limitations, mainly when they cannot answer correctly. Respondents suggested including a "degree of confidence" in the answer and reporting when the LLM is unsure.
Accuracy: Participants stressed the importance of LLMs delivering accurate and correct information consistently. 
Prompt Understanding: The ability of LLMs to better understand user input and follow instructions without much elaboration from the user. Participants desired more anticipation and less hand-holding.
Speed (fast answers): Respondents in both groups cited fast response times.
Provision of Sources: Both sectors requested that LLMs provide references or citations for the information presented.}

\textcolor{blue}{Furthermore, there were differences between the two sectors. Academia's requests focus more on LLMs providing detailed explanations, consistency, and handling complex problems, while industry participants emphasise context awareness, minimising hallucinations, and ensuring data confidentiality. }

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/feelings.png}
    \caption{Emotional responses to LLMs' wrong answers (Q8)}
    \label{fig:Q12}
\end{figure}

\subsection{Mitigations}
As recommended by some participants, Chatbots need to be transparent, this way many frustrations that are caused by the hallucinations and overconfidence of the response can be minimized, and as a consequence, it can also increase the trust towards the chatbot \cite{lee2021don}. Chatbot users can also make use of some prompting techniques to improve the indication of confidence by the chatbot \cite{xiong2023can}.
Other systematic ways to detect hallucination have been recently studied \cite{azaria2023internal, duan2024llms}. Since such approaches require access to the weights and hidden layers of the model, they can only be applied to white-box LLMs such as BERT.






\definecolor{lightpink}{rgb}{1,0.8,0.8}
\definecolor{lightblue}{rgb}{0.8,0.88,1}

\setlength{\arrayrulewidth}{0.3mm} % Width of table borders
\renewcommand{\arraystretch}{1.3}  % Increase row height for readability


\begin{table*}[!ht]
\centering
\begin{tabular}{|p{0.48\textwidth}|p{0.48\textwidth}|}
    \hline
    \cellcolor{lightpink}\textbf{Improvements expected from industry} & \cellcolor{lightblue}\textbf{Improvements expected from academia} \\
    \hline
    \begin{itemize}
        \item Reduced hallucination
        \item Context awareness (e.g., the entire project and its dependencies)
        \item To better follow instructions
        \item Realistic answers
        \item Concise answers, examples only under request
        \item Asking questions to the user if needed
        \item Guidance to create prompts
        \item Better understanding of user needs without much user elaboration
        \item Correct answers
        \item Accuracy
        \item To keep the chat history in memory
        \item Reasoning of provided answers
        \item Increased analytical capacity
        \item Sources
        \item Transparency, e.g., reporting when unable to answer
        \item Not apologizing
        \item To offer multiple answers
        \item Fast answers
        \item To ensure confidentiality of the provided data in the prompt
    \end{itemize} 
    & 
    \begin{itemize}
        \item Transparency, e.g., reporting when unable to answer correctly, degree of confidence in provided answer
        \item Integrated feedback
        \item Consistency
        \item Better prompt understanding
        \item Better explanations of answers
        \item Accuracy
        \item To provide references
        \item Up to date
        \item Longer memory
        \item Information about risks
        \item To ask questions back about what details are required in the answers
        \item Fast answers
        \item Social skills like humans
        \item Better ability to solve mathematical problems
        \item To remember when an answer is wrong so it is not repeated later
    \end{itemize} \\
    \hline
\end{tabular}
\caption{Q 12}
    \label{tab: q12}
\end{table*}



\section{Implication} 
% recommendations for HCI engineers, or robots designers.

